Extended Bayesian Estimation for In-flight Calibration of Space-based Instruments

The ongoing calibration of space-based instruments is essential to ensure accurate measurements of physical quantities such as photon flux. The goal is to obtain a unified photon-flux measurement of a single astronomical source using data obtained with multiple instruments. Calibration involves in-flight adjustments to address discrepancies arising from instrument-specific variations. Taking a statistical approach, we extend a previously proposed additive log-Normal hierarchical model with half-variance correction based on a multiplicative physical model for photon counts. The newly proposed Bayesian hierarchical model can leverage domain-specific priors to account for correlated passbands and integrate information across different instruments, sources, and passbands effectively. The model is fitted using Markov chain Monte Carlo and can provide uncertainty quantification for instrument- and source-specific parameter estimation. Moreover, we obtain valid inferences for other structural parameters of the physics model. We use data derived from Chandra and XMM-Newton X-ray observatories to illustrate the proposed inference procedure.

==> packages.tex <==
% === Font & Line Spacing ===
\usepackage{setspace}
\doublespacing
%\usepackage{times}

% === Page Geometry ===
%\geometry{letterpaper, top=2.54cm, bottom=2.54cm, left=3.175cm, right=3.175cm, marginparwidth=1.75cm}

% === Math & Theorems ===
\usepackage{amsmath, amssymb, amsfonts, amsthm}
\newtheorem{lemma}{Lemma}
\newtheorem{result}{Result}
\newtheorem{proposition}{Proposition}

% === Figures, Tables, Colors, Formatting ===
\usepackage{graphicx}
\usepackage{float}
\usepackage{xcolor}
\usepackage{bm}
\usepackage{subcaption}
\usepackage{multirow, multicol}
\usepackage{enumerate, enumitem}
\usepackage{paracol}
\usepackage{indentfirst} % Indent first paragraph after section


% === Bibliography ===
\usepackage[authoryear]{natbib} % use [authoryear] if preferred

% === Appendix Tools ===
\usepackage{appendix}

% === Hyperlinks ===
\usepackage[colorlinks=true, allcolors=blue]{hyperref}
\usepackage{ragged2e}
% === Chapter Title Spacing Patch ===

